On Using Machine Learning to Identify Knowledge in API Reference Documentation

Using API reference documentation like JavaDoc is an integral part of software development. Previous research introduced a grounded taxonomy that organizes API documentation knowledge in 12 types, including knowledge about the Functionality, Structure, and Quality of an API. We study how well modern text classification approaches can automatically identify documentation containing specific knowledge types. We compared conventional machine learning (k-NN and SVM) and deep learning approaches trained on manually annotated Java and .NET API documentation (n = 5,574). When classifying the knowledge types individually (i.e., multiple binary classifiers) the best AUPRC was up to 87%. The deep learning and SVM classifiers seem complementary. For four knowledge types (Concept, Control, Pattern, and Non-Information), SVM clearly outperforms deep learning which, on the other hand, is more accurate for identifying the remaining types. When considering multiple knowledge types at once (i.e., multi-label classification) deep learning outperforms na\"ive baselines and traditional machine learning achieving a MacroAUC up to 79%. We also compared classifiers using embeddings pre-trained on generic text corpora and StackOverflow but did not observe significant improvements. Finally, to assess the generalizability of the classifiers, we re-tested them on a different, unseen Python documentation dataset. Classifiers for Functionality, Concept, Purpose, Pattern, and Directive seem to generalize from Java and .NET to Python documentation. The accuracy related to the remaining types seems API-specific. We discuss our results and how they inform the development of tools for supporting developers sharing and accessing API knowledge. Published article: https://doi.org/10.1145/3338906.3338943

==> 2_background.tex <==
\section{Background and Definitions}
\label{sec:background}
This section summarizes the knowledge types identified by Maalej and Robillard~\cite{MR13} and provides the definitions to understand our approach based on deep learning.
% One of the earliest automated approaches to classify the knowledge types in JAVA APIs reference documentation was proposed by Metkar and Kamalapur (2014). They introduced an automated system based on Natural Language Processing (NLP) to categorize the knowledge using pattern-based Information Retrieval (IR) techniques. Robillard and Chhetri (2015) proposed a recommander system which extracts the most important pieces of information from the APIs documentation based on IR techniques and supports the developers in understanding how to use an API by recommending the knowledge items related to that API during the development. Eventually, Kumar and Devanbu (2016) introduced a model based on Support Vector Machines (SVM) to perform the knowledge categorization in Python reference documents.
\subsection{Knowledge types in API reference documentation}
Maalej and Robillard~\cite{MR13} performed a throughout investigation of the JDK and .NET API reference documentation.
The authors proposed a validated taxonomy of knowledge types based on grounded theory approach and literature review.  
The coding of the sampled 5,574 documentation units involved 17 experienced coders for an estimated effort of 279 person-hours.
The reported median inter-coder agreement was above 80\%.
The final judgment was performed following a rigorous disagreement reconciliation process.
The taxonomy of knowledge types is reported in \Cref{tbl:taxonomy}.
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
    \begin{table}[!ht]
        \centering
        \caption{Knowledge types in reference documentation after Maalej and Robillard~\cite{MR13}. }
        \begin{tabu} to \linewidth {lX}
        \toprule
        \multicolumn{1}{c}{Knowledge Type} & \multicolumn{1}{c}{Description}                                                    \\ \midrule
        Functionality                                     & Describes the capabilities of the API, and what happens when it is used.           \\
        \rowcolor[HTML]{EFEFEF} 
        Concept                                           & Explains terms used to describe the API behavior or the API implementation.       \\
        Directive                                         & Describe what the user is allowed (not allowed) to do with the API.                \\
        \rowcolor[HTML]{EFEFEF} 
        Purpose                                           & Explains the rationale for providing the API or for a design decision.             \\
        Quality                                           & Describes non-functional attributes of the API, including its implementation.      \\
        \rowcolor[HTML]{EFEFEF} 
        Control                                           & Describes how the API manages the control-flow and sequence of calls.              \\
        Structure                                         & Describes the internal organization of API elements including their relationships. \\
        \rowcolor[HTML]{EFEFEF} 
        Pattern                                           & Explains how to get specific results using the API.                              \\
        Example                                           & Provides code examples about the usage of the API.                                 \\
        \rowcolor[HTML]{EFEFEF} 
        Environment                                       & Describes the environment in which the API is used.                                \\
        Reference                                         & Pointers to external documents.                                                    \\
        \rowcolor[HTML]{EFEFEF} 
        Non-information                                   & Uninformative, boilerplate text.                                                   \\ \bottomrule
        \end{tabu}
        \label{tbl:taxonomy}
 \end{table}
\subsection{Long Short-Term Memory Networks}
%\davide{Ali, please complete this section.}
%\ali{Davide, should I add more about lstm?}
\begin{figure}
    \centering
    \includegraphics[width=.35\textwidth]{fig/lstm_cell_2.jpg}
    \caption{A single \lstm recurrent module containing input output, memory, and forget gates.}
    \label{fig:memory}
\end{figure}
Deep learning has recently brought substantial improvements in the field of machine vision and natural language processing (NLP)~\cite{DY14}.
We use \lstm to solve a multi-label classification problem---\ie~assigning a set of knowledge types to an API document.
\lstm is an extension of Recurrent Neural Networks (\rnn) which utilizes several gates and a memory cell in the recurrent module to alleviate the vanishing gradient problem and to handle more efficiently the long-term dependencies between the features~\cite{HS17}.  

We provide the intuitions behind each gate to clarify their functionality and how they support the classification of documents based on the knowledge types (see~\Cref{fig:memory}). 
The core component of \lstm is a memory cell which stores the information related to the past steps. 
At each step of the training, the network predicts the output based on the new input, the previous state of the other hidden layers of the \rnn, and the current state of the memory cell. 
The role of the gates is to learn how to modify the memory cell to enhance the prediction accuracy. 

The \textit{forget gate} ($\mathit{f_t}$) processes the information from the previous hidden state layer ($\mathit{h_{t-1}}$) and the current input ($X_t)$ to decide what should be discarded from the previous state of the memory cell ($\mathit{C_{t-1}}$). 
The \textit{input gate} ($\mathit{i_t}$) is responsible for selecting new information from the input ($\mathit{X_t}$) that should be stored in the cell state. 
The third gate is called \textit{output gate} ($\mathit{o_t}$) and decides which part of the currently available information in the memory cell should be used to produce the final output ($\mathit{h_t}$).   
